Residual Descent Differential Dynamic Game (RD3G) -- A Fast Newton Solver for Constrained General Sum Games

We present Residual Descent Differential Dynamic Game (RD3G), a Newton-based solver for constrained multi-agent game-control problems. The proposed solver seeks a local Nash equilibrium for problems where agents are coupled through their rewards and state constraints. We compare the proposed method against competing state-of-the-art techniques and showcase the computational benefits of the RD3G algorithm on several example problems.

==> derivation.tex <==
\label{appendix:der}
We are interested in solving the following problem:
\begin{subequations}
\begin{align}
&u^{i*} = \underset{u^i}{\arg \min}J^i(x,u^i) \\
\textrm{s.t.  } &f^i_k(x^i_k, u^i_k) = x_{k+1}^i, 
    \quad\forall k \in [0..T-1], \forall i\in [1..N]\\
&h_k(x^i_k, x^j_k) \leq 0 
    \quad \forall i\neq j, i,j \in [1..N], \forall k\in [1..T]\\
\textrm{where  } &J^i(x,u^i) = \sum_{k=0}^{T-1} J_k^i(x_k, u^i_k) + \phi^i(x_T)
\end{align}
\end{subequations}

Let
\begin{align}
L_k^i(x_k, u_k^i, \lambda^i_k, \mu^i_k) = J_k^i(x_k, u_k^i) + (\lambda^i_k)^\T [f_k^i(x_k,u_k^i) - x^i_{k+1}] \nonumber \\
+ \sum_{j\in H^+_{i,k}} \mu^{i,j}_kh(x_k^i, x_k^j) + \sum_{j\in H^-_{i,k}} B(h(x_k^i, x_k^j))
\end{align}
and
\begin{align}
\mathcal{L}^i(x, u^i, \lambda^i, \mu^i) = \sum_{k=1}^{T-1} L_k^i + J_0^i(x_0^i, u_0^i) + \lambda_0^{i,\T} [f_0^i(x_0^i, u_0^i) - x_1^i] \nonumber \\
+ \phi^i(x^i_T, 0) + \sum_{j\in H^+_{i,T}} \mu^{i,j}_T h(x^i_T, x^j_T) + \sum_{j \in H^-_{i,T}} B(h(x^i_T, x^j_T))
\end{align}

Then the necessary KKT conditions for optimality is:
\begin{subequations}
\begin{align}
\textrm{Primal: }&    \pp{\mathcal{L}^i}{x}=0, \pp{\mathcal{L}^i}{u^i}=0 \\
\textrm{Dual: }&   f_k^i(x_k^i, u_k^i) - x^i_{k+1} = 0, \quad\forall k\in[0..T-1] \\
&h(x^i_k, x^j_k)=0, \quad\forall j\in H^+_{i,k}, \quad\forall k\in[1..T]
\end{align}
\end{subequations}
which need to be satisfied by all agents $i\in [1..N]$

Denote 
\begin{equation}
\begin{split}
F^i = [f_0^i(x_0^i, u_0^i) - x^i_{1},f_1^i(x_1^i, u_1^i) - x^i_{2},\dots,\\
f_{T-1}^i(x_{T-1}^i, u_{T-1}^i) - x^i_{T}],
\end{split}
\end{equation}
and $h^{i,+} = [h(x^i_k, x^j_k), \forall j \in H^+_{i,k} \forall k \in [1..T]]$

We define the residual to be
\begin{equation}
    r^i(x,u^i,\lambda^i, \mu^i) = [\pp{\mathcal{L}^i}{x},\pp{\mathcal{L}^i}{u^i},F^i, h^{i,+}]
\end{equation}
and let the concatenated residual for all agents be $r = [r^1, r^2, \dots, r^N]$.

The dimension fo each variable is: $x\in R^{TNn}, u\in R^{TNm}, \lambda\in R^{TNn}, \mu \in R^{TNN}$

\subsection{Derivatives}
Our goal is to find $\nabla r$, which is assembled from many blocks of separate jacobian matrices. First we find the first order derivative $\pp{\mathcal{L}^i}{x}, \pp{\mathcal{L}^i}{u}$. To keep our notation simple, we implicitly assume $j\neq i$.
% \mathcal{L}^i, first order der
\begin{align}
\mathcal{L}^i(x, u^i,& \lambda^i, \mu^i)\\
={}& \sum_{k=1}^{T-1} L_k^i + J_0^i(x_0, u_0^i) + (\lambda_0^i)^\T [f_0^i(x_0^i, u_0^i) - x_1^i] \nonumber \\
&+ \phi^i(x_T, 0) + \sum_{j\in H^+_{i,T}} \mu^{i,j}_T h(x^i_T, x^j_T) \nonumber \\
&+ \sum_{j \in H^-_{i,T}} B(h(x^i_T, x^j_T))\\
\pp{\mathcal{L}^i}{x^i_k} ={}& \\
  ={}& \pp{L^i_k}{x^i_k} + (-\lambda^i_{k-1})^\T \quad (1\leq k \leq T-1])\\
 ={}& (-\lambda^i_{T-1})^\T + \pp{\phi^i}{x^i_T} + \sum \mu^{i,j}_{\T} \pp{h}{x^i_T} \nonumber \\
 &+ \sum \pp{B \circ h}{x^i_T} \quad (k=T)\\
\pp{\mathcal{L}^i}{x^j_k} ={}& \red{\pp{J^i_k}{x^j_k}} +  \sum\mu^{i,j}_k \pp{h}{x^j_k} + \sum  \pp{B\circ h}{x^j_k} \quad (1 \leq k \leq T-1)\\
={}& \pp{\phi^i}{x^j_T} + \sum\mu^{i,j}_k \pp{h}{x^j_k} + \sum  \pp{B\circ h}{x^j_k} \quad (k = T) \\
\pp{\mathcal{L}^i}{u^i_k} ={}& \pp{J^i_k}{u^i_k} + (\lambda^i_k)^\T \pp{f^i_k}{u^i_k} \\
\end{align}

The second-order derivatives, which compose $\nabla r$ are:
\nick{we ignore second order derivative for dynamics $f()$}

For $\pp{\mathcal{L}^i}{x}$
\begin{align}
&\ppp{\mathcal{L}^i}{x^i_k}{x^i_k} = \ppp{L^i_k}{x^i}{x^i} \\
&= \ppp{J^i_k}{x^i_k}{x^i_k} + (\lambda^i_k)^\T \ppp{f^i_k}{x^i_k}{x^i_k} + \sum \mu^{i,j}_k\ppp{h}{x^i_k}{x^i_k} \nonumber \\
&\quad + \sum \ppp{B \circ h}{x^i_k}{x^i_k}, \quad (1 \leq k \leq T-1)\\
&= \ppp{\phi^i}{x^i_k}{x^i_k} +  \sum \mu^{i,j}_k\ppp{h}{x^i_k}{x^i_k} + \sum \ppp{B \circ h}{x^i_k}{x^i_k}, \quad (k = T)\\
&\ppp{\mathcal{L}^i}{x^i_k}{x^j_k} = \ppp{L^i_k}{x^i_k}{x^j_k} \\
&=\red{\ppp{J^i_k}{x^i_k}{x^j_k}} + (\lambda^i_k)^\T \ppp{f^i_k}{x^i_k}{x^j_k} + \sum \mu^{i,j}_k\ppp{h}{x^i_k}{x^j_k} \nonumber \\
&\quad + \sum \ppp{B \circ h}{x^i_k}{x^j_k}, \quad (1\leq k \leq T-1) \\
&=\ppp{\phi^i_k}{x^i_k}{x^j_k} + (\lambda^i_k)^\T \ppp{f^i_k}{x^i_k}{x^j_k} + \sum \mu^{i,j}_k\ppp{h}{x^i_k}{x^j_k} \nonumber \\
&\quad + \sum \ppp{B \circ h}{x^i_k}{x^j_k}, \quad ( k = T) \\
&\ppp{\mathcal{L}^i}{x^i_k}{u^i_k} = \ppp{J^i_k}{x^i_k}{u^i_k}\\
&\ppp{\mathcal{L}^i}{x^i_k}{\lambda^i_{k-1}} = - I, \quad k=[1..T]\\
&\ppp{\mathcal{L}^i}{x^i_k}{\lambda^i_k} = \pp{f^i_k}{x^i_k}^\T, \quad k=[1..T-1]\\
&\ppp{\mathcal{L}^i}{x^i_k}{\mu^{i,j}_k} = \ppp{L^i_k}{x^i_k}{\mu^{i,j}_k} = \pp{h(x^i_k,x^j_k)}{x^i_k} \mathbf{1}(j\in H^+_{i,k})\\
\end{align}

% dl/dxj
\begin{align}
&\red{\ppp{\mathcal{L}^i}{x^j_k}{x^j_k} = \ppp{L^i_k}{x^j}{x^j} }\\
&= \ppp{J^i_k}{x^j_k}{x^j_k} + (\lambda^i_k)^\T \ppp{f^i_k}{x^j_k}{x^j_k} + \sum \mu^{i,j}_k\ppp{h}{x^j_k}{x^j_k} \nonumber \\
&\quad + \sum \ppp{B \circ h}{x^j_k}{x^j_k}, \quad (1 \leq k \leq T-1)\\
&\ppp{\mathcal{L}^i}{x^j_k}{\mu^{i,j}_k} = \ppp{L^i_k}{x^j_k}{\mu^{i,j}_k} = \pp{h(x^i_k,x^j_k)}{x^j_k} \mathbf{1}(j\in H^+_{i,k})
\end{align}

For $\pp{\mathcal{L}^i}{u}$
\begin{align}
&\ppp{\mathcal{L}^i}{u^i_k}{u^i_k} = \ppp{J^i_k}{u^i_k}{u^i_k} + (\lambda^i_k)^\T \ppp{f^i_k}{u^i_k}{u^i_k}\\
&\ppp{\mathcal{L}^i}{u^i_k}{\lambda^i_k} =  (\pp{f^i_k}{u^i_k})^\T 
\end{align}

The derivatives are trivial for $F^i,h^{i,+}$.

The supporting derivatives that appeared previously are listed below
% L, first order der, not used
\begin{align}
L_k^i(x_k,& u_k^i, \lambda^i_k, \mu^i_k) \\
={}& J_k^i(x_k, u_k^i) + (\lambda^i_k)^\T [f_k^i(x_k^i,u_k^i) - x^i_{k+1}] \nonumber \\
&+ \sum_{j\in H^+_{i,k}} \mu^{i,j}_kh(x_k^i, x_k^j) + \sum_{j\in H^-_{i,k}} B(h(x_k^i, x_k^j))\\
\pp{L^i_k}{x^i_k} ={}& \pp{J^i_k}{x_k^i} + (\lambda^i_k)^\T [\pp{f^i_k}{x^i_k}] + \sum \mu_k^{i,j} \pp{h}{x^i_k} + \sum \dd{B}{h} \pp{h}{x^i_k}\\
\pp{L^i_k}{x^j_k} ={}& \pp{J^i_k}{x_k^j} +\sum \mu_k^{i,j} \pp{h}{x^j_k} + \sum \dd{B}{h} \pp{h}{x^j_k}\\
\pp{L^i_k}{u^i_k} ={}& \pp{J^i_k}{u^i_k} + (\lambda^i_k)^\T \pp{f^i_k}{u^i_k}\\
\pp{L^i_k}{\mu^{i,j}_k} ={}& h(x^i_k,x^j_k) \mathbf{1}(j\in H^+_{i,k})
\end{align}

% Barrier function
\begin{align}
B(h(x^i,x^j)) ={}& - \rho^{-1} \log(-h(x^i,x^j)) \\
\dd{B}{h} ={}& -\rho^{-1} h^{-1} \\
\pp{B \circ h}{x^i} ={}& \dd{B}{h}\pp{h}{x^i}\\
\ppp{B\circ h}{x^i}{x^j} ={}& -\frac{1}{\rho h} [-\ppp{h}{x^i}{x^j} + \frac{1}{h} \ppp{h}{x^i}{x^j}]
\end{align}

The remaining derivatives for $f,J$ are application specific.

\begin{comment}
Dynamics for examples:
Car collision:
\begin{align}
J(x,u^i) ={}& (x-x_r)^\T Q_r (x-x_r) + x^\T Q x + u^\T R u ]]\\
\pp{J}{x} ={}& 2(x-x_r)^\T Q_r + 2 x^\T Q\\
\ppp{J}{x}{x} ={}& 2Q_r + 2Q
\end{align}
\begin{align}
h(x_i,x_j) ={}& (x^i-x^j)^\T Q_h (x^i-x^j) + d_{\textrm{min}}^2\\
Q_h ={}& \textrm{diag}(-1,-1,0,0)\\
\pp{h}{x^i} ={}& s (x^i-x^j)^\T Q_h
\end{align}
\end{comment}

